Cross-dimensional Weighting for Aggregated Deep Convolutional Features

We propose a simple and straightforward way of creating powerful image representations via cross-dimensional weighting and aggregation of deep convolutional neural network layer outputs. We first present a generalized framework that encompasses a broad family of approaches and includes cross-dimensional pooling and weighting steps. We then propose specific non-parametric schemes for both spatial- and channel-wise weighting that boost the effect of highly active spatial responses and at the same time regulate burstiness effects. We experiment on different public datasets for image search and show that our approach outperforms the current state-of-the-art for approaches based on pre-trained networks. We also provide an easy-to-use, open source implementation that reproduces our results.

==> fig/approach_figure.tex <==
\begin{figure}
\newcommand{\myGlobalTransformation}[2]
{
    \pgftransformcm{1}{0}{0.4}{0.5}{\pgfpoint{#1cm}{#2cm}}
%     \pgftransformcm{0.4}{0.5}{1}{1}{\pgfpoint{#1cm}{#2cm}}

}

% draw a 4x4 helper grid in 3D
% Input: point of origins x and y coordinate and additional drawing-parameters
\newcommand{\gridThreeD}[3]
{
    \begin{scope}
        \myGlobalTransformation{#1}{#2};
        \draw [#3,step=2cm] grid (8,8);
    \end{scope}
}

\tikzstyle myBG=[line width=3pt,opacity=1.0]

% draws lines with white background to show which lines are closer to the
% viewer (Hint: draw from bottom up and from back to front)
%Input: start and end point
\newcommand{\drawLinewithBG}[2]
{
    \draw[white,myBG]  (#1) -- (#2);
    \draw[black,very thick] (#1) -- (#2);
}

% draws all horizontal graph lines within grid
\newcommand{\graphLinesHorizontal}
{
    \drawLinewithBG{1,1}{7,1};
    \drawLinewithBG{1,3}{7,3};
    \drawLinewithBG{1,5}{7,5};
    \drawLinewithBG{1,7}{7,7};
}

% draws all vertical graph lines within grid
\newcommand{\graphLinesVertical}
{
    %swaps x and y coordinate (hence vertical lines):
    \pgftransformcm{0}{1}{1}{0}{\pgfpoint{0cm}{0cm}}
    \graphLinesHorizontal;
}

\newcommand{\gridcolor}{black!60}

% \begin{tikzpicture}[scale=.8, rotate=45]
\begin{tikzpicture}[scale=.6]

    %draws helper-grid:
    \begin{scope}[rotate=-90]
    \gridThreeD{0}{0}{\gridcolor};
    \gridThreeD{0}{1.75}{\gridcolor};
    \gridThreeD{0}{5.25}{\gridcolor};
	\end{scope}
%     %draws lower graph lines and those in z-direction:
%     \begin{scope}
%         \myGlobalTransformation{0}{0};
%         \graphLinesHorizontal;

%         %draws all graph lines in z-direction (reset transformation first!):
%         \foreach \x in {1,3,5,7} {
%             \foreach \y in {1,3,5,7} {
%                 \node (thisNode) at (\x,\y) {};
%                 {
%                     \pgftransformreset
%                     \draw[white,myBG]  (thisNode) -- ++(0,4.25);
%                     \draw[black,very thick] (thisNode) -- ++(0,4.25);
%                 }
%             }
%         }
%     \end{scope}

\end{tikzpicture}
\caption{The best fig in the world}
\end{figure}

==> tex/algorithms.tex <==
%-------------------------------------------------------------------------
\begin{algorithm}[t]

\DontPrintSemicolon
\SetFuncSty{textsc}
\SetDataSty{emph}
\newcommand{\commentsty}[1]{{\color{green!50!black}#1}}
\SetCommentSty{commentsty}

\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKwFunction{norm}{norm}
\SetKwFunction{whiten}{whiten}
%\SetKwFunction{sum}{sum}
% Commenting this out -- it causes sum to puke elsewhere.
\SetKwFunction{zeros}{zeros}

\Input{3d feature tensor $\cX = \{\cX_1, \ldots, \cX_K \}$, \\ pre-trained whitening parameters $W$, \\ final feature dimensionality $K^{\prime}$}
\Output{$K^{\prime}$-dimensional \SuP feature vector $\cF = \{ f_1, \ldots, f_K\}$}
\BlankLine

% $\cK \gets \emptyset$ \tcp*{set of components to keep}
% \Sort $\cC$ such that $i \leq k \to \pi_i \geq \pi_k$ for $i,k \in \cC$
% 		\tcp*{re-order components $i$\ldots}
% \ForEach(\tcp*[f]{\ldots in descending order of $\pi_i$}){$i \in \cC$}
{$ \cF =$ zeros($K$) \tcp*{initialize}}

\ForEach(\tcp*[f]{for each channel}){$k \in K$}
{
	{$f_k = sum( sum( \cX, axis=0), axis=0) $}
% 	\If(\tcp*[f]{compute $\rho_{i,\cK}$ by~(\ref{eq:rho})})
% 		{$\rho_{i,\cK} \geq \tau$}
% 		{$\cK \gets \cK \cup i$ \tcp*{keep $i$ if it does not overlap with $\cK$}}
}

{$\cF$ = norm($\cF$, L2) \tcp*{L2-normalize}}
{$\cF$ = whiten($\cF$, $W$) \tcp*{whiten}}
{$ \cF$ = norm($\cF$, L2) \tcp*{L2-normalize again}}
{$ \cF$ = PCA($\cF$, $K^{\prime}$) \tcp*{dim. reduction}}
\caption{\SuP Feature Extraction}
\label{alg:sup}
\end{algorithm}
%-------------------------------------------------------------------------




==> tex/deprecated_feature_weighting_channel.tex <==
\subsection{Sparsity Sensitive Channel Weighting}
\label{subsec:idf}

We now propose a method to derive a channel weighting based on the sparsity of feature maps. We expect that similar images will have similar occurrence rates for a given feature. We find the proportion of non-zero responses for channel $k$ and compute the \emph{per-channel sparsity} as follows:

\begin{equation}
\cQ_{k} = 1 - \left ( \frac{\sum_{ij} \mathbbm{1}[\matrixForChannel > 0]}{WH} \right )
\end{equation}

In Figure~\ref{fig:sparsity_correlation} we visualize the pair-wise correlation of the vectors of channel sparsities $\cQ \in \mathbb{R}^{K}$ for images in the query-set of the \emph{Paris} dataset. The query-set for the \emph{Paris} dataset contains 55 images total, 5 images each for 11 classes of Paris landmarks. We order the images by class. It is apparent that channel sparisities $\cQ$ are highly correlated for images of the same landmark and less correlated for images of different landmarks. It appears that the sparsity pattern of channels contains discriminative information.

% Let $X_k^0$ ne the zero-norm of channel $\cX_k, k \in K$, \ie the number of non-zero responses in that channel. Let vector $\cX^0 =\{ x_1^0, \ldots, x_k^0 \}$ and $\|\cX^0\| = \sum_k x_k^0$. Vector $\cX^0$ contains.......???

Since we sum-pool features $\channelsAtLocation$ over spatial locations when we derive our aggregated feature, channels with frequent feature occurrences are already strongly activated in the aggregate feature. However, infrequently occurring features could provide important signal if, for example, the feature consistently occurs though only a small number of times in images of the same class. Motivated by this insight, we devise a channel weighting scheme similar to the concept of \emph{inverse document frequency}. That is, we boost the contribution of rare features in the

\alert {
NOTE: general issue here in pivoting the use of Q as sparsity into the weights. The math is messier if you express the idf weights in terms of Q because you need to undo the "1 -". We probably need to not use sparsity but highlight the relationship in a sentence or two.

If instead

\begin{equation}
\cQ_{k} = \left ( \frac{\sum_{ij} \mathbbm{1}[\matrixForChannel > 0]}{WH} \right )
\end{equation}

then channel weights $\cI_{k}$ are

\begin{equation}
\cI_{k} = \log(( \frac{\sum_{h} \cQ_{h}}{\cQ_{k}} )
\end{equation}

Here is prior stuff expressing it as zero-norm:


If we treat the aforementioned ? in a \textit{idf} fashion we can get vector $\cI = \{ i_1, \ldots, i_k \}$, where:
\begin{equation}
i_k = \log( \frac{\|\cX^0\|}{x_k^0} ), 
\end{equation}
where $k \in K$.
}
            
% --- show weak/strong channels/filters

% --- create spatial map of strong idf channel activation, i.e. weight channels by idf weight, sum over channels, normalize - are hot locations "unique" in the image?

% --- describe account of idf weight taking locations(or is it channels? - i am confussed [yannis]) as "documents" and aggregate feature as "query" CM; could we consider aggregate features in general as an efficient alternative to indexing all locations of all images and querying with all locations of query image

---- relation with democratic aggregation? / burstiness


%------------------------------------------------------------------------------
\begin{figure}
\centering
\includegraphics[width=.8\columnwidth]{fig/non_zero_perc.png}
\vspace{-0.65cm}
\caption{The correlation of channel-wise sparsity for images in the query-set of the \emph{Paris} dataset. Images are sorted by landmark class in both dimensions.}
\label{fig:sparsity_correlation}
\end{figure}
%------------------------------------------------------------------------------


==> tex/experiments_finegrained.tex <==
\subsection{Unsupervised Fine-grained Classification}
\label{subsec:exp_finegrained}

The state-of-the-art on fine-grained classification has advanced rapidly during the last few years, with many approaches either training on or mining object parts~\cite{SiRD14, KJYL15, QJZL15}. We are mostly interested in fully unsupervised classification, \ie approaches that do not require bounding boxes or parts for either training or testing and therefore do not include in our comparisons part-based approaches~\cite{KJYL15, QJZL15} that require bounding boxes or parts for training.

Simon~\etal~\cite{SiRD14} start from a pre-trained CNN and discover part detectors in a supervised as well as unsupervised way.  In their recent paper, Gavves~\etal~\cite{GBC+15} propose learning \textit{alignments} of parts of objects using just the overall shape. They use object detectors as voters to generate object confidence saliency maps and a bundle of color Fisher Vectors for representation.

We report results on the \emph{Birds} dataset against the state-of-the-art in Table~\ref{tab:cub}. As this is a different application, we report results for all variants of our approach. We see that our weighting approaches boost performance significantly, both independently and jointly. It is worth noting that the highest performing competitors have very computationally heavy training and testing phases~\cite{SiRD14} or further require feature fusion~\cite{GBC+15}. Our approach is training- and parameter-free and independent in the number of classes.

% Iscen~\etal~\cite{ITGJ15} 
% GMP~\cite{MuPe14} 

%------------------------------------------------------------------------------
\begin{table}
\centering
\begin{tabularx}{\columnwidth}{X c c}
% \toprule
Method & $d$ & Accuracy (\%) \\
\midrule
% \hline
\supp & 128 &  34.2 \\

GMP~\cite{MuPe14} & 256 & 17.0 \\
% GMP+Color~\cite{MuPe14} & 256 & 33.3 \\
\supp & 256 &  \textbf{47.5} \\

\midrule

Iscen~\etal~\cite{ITGJ15} & 4K & 31.9\\

% CNN baseline (\cite{SiRD14}) & --- & 41.6 \\ 
% CNN baseline w. bboxes (\cite{SiRD14}) & --- & 56.0 \\ 

Gavves~\etal~\cite{GBC+15} & --- & 53.6 \\
Simon~\etal~\cite{SiRD14} & --- & 53.8 \\

\midrule

\Sup & 512 & 50.2 \\
\Sup+\IDF & 512 &  53.9 \\
\Sup+\SCM & 512 &  55.5 \\
\supp & 512 &  \textbf{56.5} \\
% \bottomrule
% \hline
% \vspace{.05cm}
\end{tabularx}
\caption{Accuracy for unsupervised fine-grained classification on CUB-2011 Birds dataset.}
\label{tab:cub}
\end{table}
%------------------------------------------------------------------------------





